Optimizing Mixed Autonomy Traffic Flow With Decentralized Autonomous Vehicles and Multi-Agent RL

We study the ability of autonomous vehicles to improve the throughput of a bottleneck using a fully decentralized control scheme in a mixed autonomy setting. We consider the problem of improving the throughput of a scaled model of the San Francisco-Oakland Bay Bridge: a two-stage bottleneck where four lanes reduce to two and then reduce to one. Although there is extensive work examining variants of bottleneck control in a centralized setting, there is less study of the challenging multi-agent setting where the large number of interacting AVs leads to significant optimization difficulties for reinforcement learning methods. We apply multi-agent reinforcement algorithms to this problem and demonstrate that significant improvements in bottleneck throughput, from 20\% at a 5\% penetration rate to 33\% at a 40\% penetration rate, can be achieved. We compare our results to a hand-designed feedback controller and demonstrate that our results sharply outperform the feedback controller despite extensive tuning. Additionally, we demonstrate that the RL-based controllers adopt a robust strategy that works across penetration rates whereas the feedback controllers degrade immediately upon penetration rate variation. We investigate the feasibility of both action and observation decentralization and demonstrate that effective strategies are possible using purely local sensing. Finally, we open-source our code at https://github.com/eugenevinitsky/decentralized_bottlenecks.

==> mathimport.tex <==
% Fix appearance of quotes
\usepackage{csquotes}
\MakeOuterQuote{"}

\usepackage{url}

% Bibliography options
% See http://sites.stat.psu.edu/~surajit/present/bib.htm
% \usepackage{natbib} % includes \citet
% \renewcommand{\cite}{\citep}


\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{verbatim}
\usepackage{listings}
\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n} % However for large sigmas we want the Computer Modern symbol
\renewcommand{\ttdefault}{cmtt}
\usepackage{array}
% \usepackage{multirow}
\usepackage{color}
% \usepackage{clrscode4e}
\usepackage{xspace} % xspace takes care of the \@ after a capitalized word before a period.
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{caption}
% \usepackage{subcaption}
\usepackage{fancyhdr}
\usepackage{booktabs}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{wrapfig}
% \usepackage{centernot}

%% TODOnotes settings
\usepackage[color={red!100!green!33},colorinlistoftodos]{todonotes} % http://www.tex.ac.uk/tex-archive/macros/latex/contrib/
\presetkeys{todonotes}{inline}{}
% \renewcommand\todo[1]{}
\newcommand{\todoc}{\todo[caption={}]}
\newcommand{\todoactive}[1]{\todo[color=green!40]{Active (#1)}}


% \newcommand{\handout}[1]{\thispagestyle{empty}
%  \markboth{Handout \protect\ref{#1}: \protect\ref{#1-title}}{Handout \protect\ref{#1}: \protect\ref{#1-title}}
%  \pagestyle{myheadings}\htitle{\protect\ref{#1}}{\protect\ref{#1-title}}{\protect\ref{#1-date}}}

% Ignore hboxes overfull by 1 point or less.
\hfuzz 1pt

% Formatting parameters for floats.
\setcounter{topnumber}{3}
\renewcommand\topfraction{.7}
\setcounter{bottomnumber}{1}
\renewcommand\bottomfraction{.3}
\setcounter{totalnumber}{5}
\renewcommand\textfraction{.1}
\renewcommand\floatpagefraction{.7}
\setcounter{dbltopnumber}{2}
\renewcommand\dbltopfraction{.7}
\renewcommand\dblfloatpagefraction{.7}

% % default style assignments
% \def\UrlBreaks{\do\-\do\.\do\@\do\\\do\/\do\!\do\_\do\|\do\;\do\>\do\]%
%  \do\)\do\,\do\?\do\'\do\+\do\=\do\#}%
% \def\UrlBigBreaks{\do\:\do@url@hyp}%
% \def\UrlNoBreaks{\do\(\do\[\do\{\do\<}%
% % any ordinary characters that aren't usually:
% \def\UrlOrds{\do\*\do\~\do\'\do\"}%
% \def\UrlSpecials{\do\ {\Url@space}\do\%{\Url@percent}\do\^^M{\Url@space}%
%    \Url@force@Tilde}% package option may force faked text-ascii-tilde

% Some hacks to make HTML happier.
\newcommand{\vskipargs}[1]{\vskip #1}
\newcommand{\newproc}{\hrule\vskipargs{1ex plus 0.1ex minus 0.1ex}}

% Tilde for webstuff
\newcommand{\webtilde}{\raisebox{-.8ex}\~}

% Comment out chunks.
\newcommand{\punt}[1]{}

% Footnote commands.
\newcommand{\footnotenonumber}[1]{{\def\thempfn{}\footnotetext{#1}}}
\newcommand{\footnotetight}[1]{\footnote{\renewcommand\baselinestretch{1}\footnotesize #1}}

%% Math Stuff, Symbols

% From probability-distributions.tex
\def\cs#1{\hbox{\tt\string#1}}%
\def\var#1{\ifmmode#1\else$#1$\fi}% usual variable
\def\vari#1{\ifmmode\hbox{\it#1}\else{\it#1}\fi}% variable in italic
\def\vartype#1{\ifmmode\hbox{\tt#1}\else{\tt#1}\fi}% variable type

% Number sets.
\newcommand{\reals}         {\mathbb{R}}%\mathbbm{R}}    %% bbm seems to produce type 3 fonts
\newcommand{\RNN}         {\R_{\geq0}}
\newcommand{\integers}      {\mathbf{Z}}
\newcommand{\naturals}      {\mathbf{N}}
\newcommand{\rationals}     {\mathbf{Q}}
\newcommand{\complex}       {\mathbf{C}}

% Useful shorthands.

\newcommand{\lgg}       {\lg\lg}
\newcommand{\lggg}      {\lg\lg\lg}
\newcommand{\lgggg}     {\lg\lg\lg\lg}

\newcommand{\lnn}       {\ln\ln}
\newcommand{\lnnn}      {\ln\ln\ln}
\newcommand{\lnnnn}      {\ln\ln\ln\ln}

\newcommand{\norm}[1]       {\left\| #1\right\|}
\newcommand{\set}[1]        {\left\{ #1 \right\}}
\newcommand{\abs}[1]        {\left| #1\right|}
\newcommand{\card}[1]       {\left| #1\right|}
\newcommand{\floor}[1]      {\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]       {\left\lceil #1 \right\rceil}
\newcommand{\ang}[1]        {\ifmmode{\left\langle #1 \right\rangle}
                 \else{$\left\langle${#1}$\right\rangle$\xspace}\fi}
                        % the \if allows use outside mathmode,
                    % but may swallow following space there!
\newcommand{\sbrace}[1]{\left[#1\right]}
\newcommand{\cbrace}[1]{\left\{#1\right\}}
\newcommand{\paren}[1]      {\left( #1 \right)}
\newcommand{\prob}[1]       {\Pr\left\{ #1 \right\}}
\newcommand{\expect}[1]     {{\rm E}\left[ #1 \right]}
\newcommand{\expectsq}[1]   {{\rm E}^2\left[ #1 \right]}
\newcommand{\variance}[1]   {{\rm Var}\left[ #1 \right]}
\renewcommand{\choose}[2]   {{\dbinom{#1}{#2}}}

\newcommand{\goesto}     {\rightarrow}


\def\pmod#1{\allowbreak\mkern12mu({\rm mod}\,\,#1)}

\newcommand{\matx}[2]       {\left(\!\!\!\begin{array}{*{#1}{c}}#2\end{array}\!\!\!\right)}
\newcommand{\Adj}       {\mathop{\rm Adj}\nolimits}
\newcommand{\percent}[1]    {#1\%}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WARNING some of these theorem environments are included 
% by default from beamer, I think
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{claim}{Claim}
%\newtheorem{corollary}{Corollary}
%\newtheorem{principle}{Principle}
%\newtheorem{theorem}        {Theorem}
%\newtheorem{lemma}[theorem] {Lemma}
%\newtheorem{corollary}[theorem] {Corollary}
%\newtheorem{xample}     {Example}

\theoremstyle{definition}
% \newtheorem{nondefinition}[theorem]{Non-Definition}
% \newtheorem{exercise}[theorem]{Exercise}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{warning}[theorem]{Warning}
%\newtheorem{examples}[theorem]{Examples}
%\newtheorem{example}[theorem]{Example}
% \newenvironment{example}    {\begin{xample}\rm}{\end{xample}}

% \newenvironment{proof}      {\noindent\textsc{Proof.}\hspace{0.5em}}{\qed\par}
\def\squarebox#1{\hbox to #1{\hfill\vbox to #1{\vfill}}}
\newcommand{\qedbox}
{\vbox{\hrule\hbox{\vrule\squarebox{.667em}\vrule}\hrule}}
% \newcommand{\qed}               {\nopagebreak\mbox{}\hfill\qedbox\smallskip}
\newenvironment{proofsketch}    {\noindent\textsc{Proof Sketch.}\hspace{0.5em}}{\qed}

\newenvironment{proofidea}    {\noindent\textsc{Proof Idea.}\hspace{0.5em}}


\newcommand{\eqnref}[1]     {(\protect\ref{#1})}

\newcommand{\transpose}     {^{\mbox{\scriptsize \sf T}}}
\newcommand{\amortized}[1]  {\widehat{#1}}

% \renewcommand{\cases}[1]    {\left\{ \begin{array}{ll}#1\end{array}\right.}
\newcommand{\cif}[1]        {\mbox{if $#1$}}
\newcommand{\cwhen}[1]      {\mbox{when $#1$}}
\newcommand{\cotherw}       {\mbox{otherwise}}

%Narrow arrays
\newlength{\savearraycolsep}
\newcommand{\narrowarray}[1]{\setlength{\savearraycolsep}{\arraycolsep}\setlength{\arraycolsep}{#1\arraycolsep}}
\newcommand{\normalarray}{\setlength{\arraycolsep}{\savearraycolsep}}

% definitions and special styles

\newcommand{\defn}[1]       {{\textit{\textbf{\boldmath #1}}}}
\newcommand{\indep}       	   {\!\perp\!\!\!\perp} % Independent

% operators
\let\oldphi=\phi
\renewcommand{\phi}{\varphi}
\newcommand{\Alt}{\operatorname{Alt}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\so}{\mathfrak{so}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\vol}{\operatorname{vol}}
\newcommand{\grad}{\operatorname{grad}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\rang}{\operatorname{rang}}
\newcommand{\pr}{\operatorname{pr}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\rg}{\operatorname{rg}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\adj}{\operatorname{adj}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\cone}{\operatorname{cone}}
\newcommand{\argmin}{\operatorname{argmin}}
\newcommand{\argmax}{\operatorname{argmax}}

% Script letters
\renewcommand{\AA}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\KK}{\mathcal{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\RR}{\mathcal{R}}
\renewcommand{\SS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\WW}{\mathcal{W}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\YY}{\mathcal{Y}}
\newcommand{\ZZ}{\mathcal{Z}}

% Block letters
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\J}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\renewcommand{\L}{\mathbb{L}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\O}{\mathbb{O}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\Var}{\operatorname{Var}}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\d}{\text{d}}
\newcommand{\NS}{\text{N}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The Code environment %%%
%% The following commands are so we can automatically number and symbolically reference
%% lines.
%% The ``codelinenumber'' counter counts the current line number
%\newcounter{codelinenumber}
%% The \zeroli command zeros the line number counter
%\newcommand{\zeroli}{\setcounter{codelinenumber}0}
%% The \li command bumps the counter, outputs it, and skips some space
%% It also GLOBALLY sets the value of \@currentlabel, so that the \label
%% commands on the same line work OK.  The problem otherwise is that Latex
%% uses groups on each field of a line in tabbing mode, and this causes
%% \@currentlabel to get reset as soon as a field ends (e.g. at the \').
%% Now, the label can appear after the \\, as in
%%  \li \>\>$x\gets y$ \\ \label{li:assign-x}
%%

\def\code{\lstinline[basicstyle=\ttfamily]}

%% Labels
\newcommand{\figlabel}[1]   {\label{fig:#1}}
\newcommand{\tablabel}[1]   {\label{tab:#1}}
\newcommand{\stlabel}[1]    {\label{st:#1}}
\newcommand{\thmlabel}[1]   {\label{thm:#1}}
\newcommand{\lemlabel}[1]   {\label{lem:#1}}
\newcommand{\corlabel}[1]   {\label{cor:#1}}
\newcommand{\eqlabel}[1]    {\label{eq:#1}}
\newcommand{\ineqlabel}[1]  {\label{ineq:#1}}
\newcommand{\caselabel}[1]  {\label{case:#1}}
\newcommand{\lilabel}[1]    {\label{li:#1}}

%% References

\newcommand{\chapref}[1]    {Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]     {Section~\ref{sec:#1}}
\newcommand{\secreftwo}[2]  {Sections \ref{sec:#1} and~\ref{sec:#2}}
\newcommand{\secrefthree}[3]    {Sections \ref{sec:#1}, \ref{sec:#2}, and \ref{sec:#3}}
\newcommand{\secreffour}[4] {Sections \ref{sec:#1}, \ref{sec:#2}, \ref{sec:#3}, and~\ref{sec:#4}}
\newcommand{\appref}[1]     {Appendix~\ref{app:#1}}
\newcommand{\figref}[1]     {Figure~\ref{fig:#1}}
\newcommand{\figreftwo}[2]  {Figures \ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\tabref}[1]     {Table~\ref{tab:#1}}
\newcommand{\stref}[1]      {Step~\ref{st:#1}}
\newcommand{\strefs}[2]     {Steps~\ref{st:#1}--\ref{st:#2}}
\newcommand{\streftwo}[2]   {Steps \ref{st:#1} and~\ref{st:#2}}
\newcommand{\thmref}[1]     {Theorem~\ref{thm:#1}}
\newcommand{\thmreftwo}[2]  {Theorems~\ref{thm:#1} and~\ref{thm:#2}}
\newcommand{\lemref}[1]     {Lemma~\ref{lem:#1}}
\newcommand{\lemreftwo}[2]  {Lemmas \ref{lem:#1} and~\ref{lem:#2}}
\newcommand{\lemrefthree}[3]    {Lemmas \ref{lem:#1}, \ref{lem:#2}, and~\ref{lem:#3}}
% \newcommand{\corref}[1]     {Corollary~\ref{cor:#1}}
\renewcommand{\eqref}[1]      {Equation~(\ref{eq:#1})}
\newcommand{\eqreftwo}[2]   {Equations (\ref{eq:#1}) and~(\ref{eq:#2})}
\newcommand{\ineqref}[1]    {Inequality~(\ref{ineq:#1})}
\newcommand{\ineqreftwo}[2] {Inequalities (\ref{ineq:#1}) and~(\ref{ineq:#2})}
\newcommand{\invref}[1]     {Invariant~\ref{inv:#1}}
\newcommand{\invrefs}[2]    {Invariants \ref{inv:#1}--\ref{inv:#2}}
\newcommand{\invreftwo}[2]  {Invariants \ref{inv:#1} and~\ref{inv:#2}}
\newcommand{\defref}[1]     {Definition~\ref{def:#1}}
\newcommand{\propref}[1]    {Property~\ref{prop:#1}}
\newcommand{\caseref}[1]    {Case~\ref{case:#1}}
\newcommand{\casereftwo}[2] {Cases \ref{case:#1} and~\ref{case:#2}}
\newcommand{\liref}[1]      {line~\ref{li:#1}}
\newcommand{\Liref}[1]      {Line~\ref{li:#1}}
\newcommand{\lirefs}[2]     {lines \ref{li:#1}--\ref{li:#2}}
\newcommand{\Lirefs}[2]     {Lines \ref{li:#1}--\ref{li:#2}}
\newcommand{\lireftwo}[2]   {lines \ref{li:#1} and~\ref{li:#2}}
\newcommand{\lirefthree}[3] {lines \ref{li:#1}, \ref{li:#2}, and~\ref{li:#3}}
\newcommand{\exref}[1]      {Exercise~\ref{ex:#1}}
\newcommand{\princref}[1]   {Principle~\ref{prop:#1}}

% % Specific for CS270
\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}


